Res-Attn : An Enhanced Res-Tuning Approach with Lightweight Attention Mechanism

Res-Tuning introduces a flexible and efficient paradigm for model tuning, showing that tuners decoupled from the backbone network can achieve performance comparable to traditional methods. Existing methods commonly construct the tuner as a set of trainable low-rank decomposition matrices, positing that a low-rank subspace suffices for adapting pre-trained foundational models to new scenarios. In this work, we present an advanced, efficient tuner augmented with low-rank attention, termed Res-Attn , which also adheres to the Res-Tuning framework. Res-Attn utilizes a parallel multi-head attention module equipped with low-rank projections for query, key, and value to execute streamlined attention operations. Through training this lightweight attention module, Res-Attn facilitates adaptation to new scenarios. Our extensive experiments across a range of discriminative and generative tasks showcase the superior performance of our method when compared to existing alternatives

==> tables_arxiv/coco.tex <==
% \begin{table}[t]
% \caption{
% \textbf{Comparison of FID and efficiency on COCO2017.} Following the default settings of stable diffusion\protect\footnotemark, we sample 10k captions from the validation set for generating images of size $512^{2}$ using 50 PLMS steps with classifier-free guidance scale 3.0 and compare against the full validation set.
% }
% \label{taba:coco}
% \vspace{2pt}
% \setlength{\tabcolsep}{12pt}
% \centering\footnotesize
% \begin{tabular}{l|cccc}
% \toprule
% Method & FID & Param. (M) & Mem. (GB) & Train (Hour/Epoch) \\
% \midrule
% SD v1.5 & 15.48 & - & - & - \\
% + Full & 14.85 & 862 (100\%) & 72.77 & 1.98 \\
% \midrule
% + LoRA & 14.50 & 9.96 (1.15\%) & 61.03 & 1.42 \\
% + Adapter & 14.73 & 2.51 (0.29\%) & 54.30 & 1.30 \\
% + Prefix & 15.36 & 4.99 (0.58\%) & 64.91 & 2.20 \\
% + Prompt & 14.90 & \textbf{1.25} (0.14\%) & 63.70 & 2.17 \\
% + Res-Tuning & \textbf{13.96} & 2.54 (0.29\%) & 54.49 & 1.38 \\
% \midrule
% + Res-Tuning & \textbf{13.96} & 2.54 (0.29\%) & 54.49 & 1.38 \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \end{table}
% \footnotetext{https://huggingface.co/runwayml/stable-diffusion-v1-5} 
